PointEval: On the Impact of Pointer Analysis Frameworks

Pointer analysis is a foundational analysis leveraged by various static analyses. Therefore, it gathered wide attention in research for decades. Some pointer analysis frameworks are based on succinct declarative specifications. However, these tools are heterogeneous in terms of the underlying intermediate representation (IR), heap abstraction, and programming methodology. This situation complicates a fair comparison of these frameworks and thus hinders further research. Consequently, the literature lacks an evaluation of the strengths and weaknesses of these tools. In this work, we evaluate two major frameworks for pointer analysis, WALA and Doop, on the DaCapo set of benchmarks. We compare the pointer analyses available in Wala and Doop, and conclude that---even though based on a declarative specification---Doop provides a better pointer analysis than Wala in terms of precision and scalability. We also compare the two IRs used in Doop, i.e., Jimple from the Soot framework and IR from the Wala framework. Our evaluation shows that in the majority of the benchmarks Soot's IR gives a more precise and scalable pointer analysis. Finally, we propose a micro-benchmark \emph{PointerBench}, for which we manually validate the points-to statistics to evaluate the results of these tools.

==> sections/discussion.tex <==
%!TEX root = ../PointEval.tex
% \subsection{Threats to Validity}

In this section we discuss the limitations of our study. One of the limitations is the
code coverage during profiling of benchmark application in \emph{PointBench} to compute heap
information. Since the heap information is computed dynamically, we manually increase the code
coverage in the benchmark applications to mitigate this limitation. The benchmark
applications are small in size, and therefore it is possible to write test cases such that every path in the program is
executed without requiring any input from the user.

Another limitation of this study is the choice of the microbenchmark applications not employing new
dynamic features of Java~8 such as lambdas. To the best of our knowledge, various static analysis
frameworks are unsound with respect to these novel features~\cite{Reif2018,Rief2019}.

The evaluation of the DaCapo benchmarks may suffer from the limitations of the reflection analysis. Static reflection
analysis is often limited to conservatively assume that the
reflective calls creates objects of every subtype of the receiving variable's static type or of the type of a subsequent type cast. In contrast, dynamic analysis such as
\emph{TamiFlex}~\cite{tamiflex2011Bodden} may not resolve all reflective calls %and choose to ignore some
and hence, compromises on soundness. This results in a call-graph lacking edges for some potential
reflective calls~\cite{Reif2018} (true negatives) and consequently, results in an unsound pointer
analysis, as pointer analysis is interdependent on the call-graph construction. However, this is
another line of research and beyond the scope of this work.

==> sections/implementation.tex <==
\section{Implementation}

